Towards an accountable Internet of Things: A call for reviewability

As the IoT becomes increasingly ubiquitous, concerns are being raised about how IoT systems are being built and deployed. Connected devices will generate vast quantities of data, which drive algorithmic systems and result in real-world consequences. Things will go wrong, and when they do, how do we identify what happened, why they happened, and who is responsible? Given the complexity of such systems, where do we even begin? This chapter outlines aspects of accountability as they relate to IoT, in the context of the increasingly interconnected and data-driven nature of such systems. Specifically, we argue the urgent need for mechanisms - legal, technical, and organisational - that facilitate the review of IoT systems. Such mechanisms work to support accountability, by enabling the relevant stakeholders to better understand, assess, interrogate and challenge the connected environments that increasingly pervade our world.

==> misc.tex <==
%\section{Accountability in an automated world}
\section{A system of systems}

% Our physical environments are becoming increasingly interconnected, automated, and data-driven as the grand vision of the Internet of Things (IoT) becomes a reality. 
% Such IoT deployments might include a smart home management system which controls the temperature depending on the weather, the time, and who is currently at home; or it might be a city-wide control centre, using an array of vehicle sensors and variable road signs to automatically redirect traffic and reduce congestion.
% In both examples, these deployments comprise a range of devices collectively working together to achieve a common goal. %, and can lead to more-informed, data-driven decisions about when certain actions should be taken.


% Yet, there is more to the IoT than just the devices; the interconnected nature of these systems means that they rarely operate discretely and in isolation.
% From a technical perspective, such deployments are often a \emph{system of systems} -- a `chain' of interconnected systems comprising a wider, collective system.
% This chain might include many devices generating vast quantities of data, online services providing 

% , interconnected into the IoT deployment

% perhaps involving many devices, online services, and organisational entities. 
% In other words, an IoT deployment may include vast quantities of data, from a range of different sources (sensors, online services) 




% These systems might include a wide range of sensors generating vast quantities of data being fed into various algorithmic models


% Vast quantities of data from a wide range of sources are processed into actions or decisions.
% These may include readings from local sensors, online services, and user input, 


% These are often fed into algorithmic systems, such as machine learning (ML) models, which take the data and process it in such a way as to solve certain kinds of problems.



% The complexity of these systems-of-systems is set to increase as more and more advanced technologies are developed, deployed, interconnected, and automated, by a range of entities, and this poses significant challenges for accountability. 
% Importantly, the data flows that drive these interconnected systems are often invisible or opaque. 
% This makes it difficult to exercise oversight and to determine where something went wrong and who is responsible, or in some cases, even to identify the entities involved.











\subsection{Decision pipelines}


% Focus on ML/automation aspect. Then point out that these have consequences!



Such systems can result in decisions and actions, near-instantaneously, and at scale.
Despite their grand potential, they can and do go wrong. 
For example...
When this happens, they can result in far-reaching and cascading consequences in the real-world.


As the IoT becomes more interwoven into society, we may find ourselves increasingly reliant on devices and systems of which we have little understanding.
When these systems fail in some way and harms result, this raises significant questions about how such IoT deployments should be built.
For example, how do we know that the technologies being deployed are doing the right thing? 
Where has the data come from?
In the event that something does go wrong, how might we identify what happened in order to prevent re-occurences? 
How do we identify who is responsible -- or, in some cases, who is even involved?




\subsection{The challenge of interconnectedness}

A natural first step is to look to see what went wrong. 
However, transparency within IoT, and algorithmic systems more widely, is often challenging. 
    
Firstly, systems are becoming more complex:
    \begin{enumerate}
        \item IoT arrangements often involve converting sensor readings and other data sources into real-world actions or decisions.
        \item In this way, IoT data flow can be seen as a supply chain (diagram)
        \item Identifying where something went wrong may be challenging in itself.
    \end{enumerate}
    
Another challenge is that many entities may be involved in this supply chain. 
    \begin{enumerate}
        \item Several organisations may be providing services which are vital to the IoT deployment’s successful operation (cloud servers, storage, MLaaS, IoT APIs, etc.)
        \item Each new device/service/organisation represents a new potential point of failure
    \end{enumerate}

These services may also be an effective ``black box"
    \begin{enumerate}
        \item It may not be clear how an organisation or service is influencing a data supply chain, and what cascading effects may be associated with their use
        \item We may know that a particular MLaaS model is used, but not how it works or why it produced the decision it did. 
        \item There are not enough interventions at each step
    \end{enumerate}
    
The organisations behind these services are also becoming increasingly consolidated
    \begin{enumerate}
        \item AWS, Google, Microsoft, etc.
        \item Insights from consolidation paper
        \item Implications for resilience and corporate power
    \end{enumerate}
    
In all, there is a need for a better understanding of methods and approaches for accountability within the IoT.










% Why that's a problem
\begin{itemize}
    \item This topic is timely, as there are increased legal, regulatory, and societal concerns regarding the technologies that surround us.
    \begin{itemize}
        \item In an IoT context, the privacy of smart devices has come under intense scrutiny
        \begin{enumerate}
            \item Alexa sending private conversations to the cloud
            \item Data leakages (e.g. examples of advertising networks being called)
            \item Data breaches
            \item Smart cameras (facial recognition?) in public spaces
        \end{enumerate}
        \item As a result of data-related concerns, much has been made of the GDPR.
        \begin{itemize}
            \item The GDPR offers assurances with regard to data protection, and disincentivises bad practice through the potential for punitive actions.
            \item But, as we will discuss, it isn't a silver bullet to all accountability-related concerns.
        \end{itemize}
    \end{itemize}
\end{itemize}


\subsection{Toward accountability in technologies}
\begin{itemize}   
    \item There is a need for IoT deployments (and technology more widely) to be built with accountability in mind.
    \begin{enumerate}
        \item A broad definition of accountability (in general, and in legal contexts)
        \item How can accountability be facilitated in technology? E.g. more transparency, governance, and oversight
    \end{enumerate}
    \item 
\end{itemize}







    



